Measurement of the proton and the deuteron structure functions F2p and F2d

The proton and deuteron structure functions F2p and F2d were measured in the kinematic range 0.006<x<0.6 and 0.5<Q^2<75 GeV^2, by inclusive deep inelastic muon scattering at 90, 120, 200 and 280 GeV. The measurements are in good agreement with earlier high precision results. The present and earlier results together have been parametrised to give descriptions of the proton and deuteron structure functions F2 and their uncertainties over the range 0.006<x<0.9.

==> anmcf2_intro.tex <==
%auto-ignore
% Measurement of the proton and the deuteron structure
% functions F2p and F2d.
% NMC preprint CERN-PPE/95-138, September 4, 1995
% Submitted to Physics Letters.
% The latex file is using the epsfig.sty and rotating.sty files
% (as are readily available from this very distribution centre),
% and the f2fig.uu file which containes the tar'red, gz-
% compressed figure files, the table files and this explanatory text.
% After unpacking you should have the following: 
%   760 anmcf2_intro.tex
% 23416 nmcf2_prep.tex
%162933 f2_fig6_111.eps
%139324 f2_fig5_111.eps
% 70427 f2_fig4_b.eps
% 80199 f2_fig4_a.eps
% 43859 f2_fig3.eps
% 55270 f2_fig2_b.eps
% 46321 f2_fig2_a.eps
% 55306 f2_fig1_b.eps
% 46617 f2_fig1_a.eps
% 20647 table_h2.tex
% 20649 table_d2.tex
%

